Polynomial speedup in Torontonian calculation by a scalable recursive algorithm

Evaluating the Torontonian function is a central computational challenge in the simulation of Gaussian Boson Sampling (GBS) with threshold detection. In this work, we propose a recursive algorithm providing a polynomial speedup in the exact calculation of the Torontonian compared to state-of-the-art algorithms. According to our numerical analysis the complexity of the algorithm is proportional to $N^{1.0691}2^{N/2}$ with $N$ being the size of the problem. We also show that the recursive algorithm can be scaled up to HPC use cases making feasible the simulation of threshold GBS up to $35-40$ photon clicks without the needs of large-scale computational capacities.

==> piszkozat.tex <==
\section{Cholesky based determinant calculation}
Elszámoltam, nem jó így...
If we have a selfadjoint positive definite matrix $M$ in dimension $d$, we can decompose it in the following way: $M = L \cdot L^\dagger,$ where $L$ is a lower triangular matrix.

If we have a submatrix of $M$, it can be constructed from $L$: (indices of $M$ mean the submatrix in rows and columns, indices of $L$ mean the submatrix rowwise)
\begin{align}
    M_I = M_{i_1, i_2, \dots, i_n} = L_{i_1, i_2, \dots, i_n} \cdot L_{i_1, i_2, \dots, i_n}^\dagger \\
    \det(M_I) = 
        \left(\sum_{k=1}^{i_1} l_{i_1k}\overline{l_{i_1k}}\right)
        \left(\sum_{k=i_1+1}^{i_2} l_{i_2k}\overline{l_{i_2k}}\right)
        \dots
        \left(\sum_{k=i_{n-1}+1}^{i_n} l_{i_nk}\overline{l_{i_nk}}\right)
\end{align}
